Statistical Analysis of Interplanetary Shocks from Mercury to Jupiter

In situ observations of interplanetary (IP) coronal mass ejections (ICMEs) and IP shocks are important to study as they are the main components of the solar activity. Hundreds of IP shocks have been detected by various space missions at different times and heliocentric distances. Some of these are followed by clearly identified drivers, while some others are not. In this study, we carry out a statistical analysis of the distributions of plasma and magnetic parameters of the IP shocks recorded at various distances to the Sun. We classify the shocks according to the heliocentric distance, namely from 0.29 to 0.99 AU (Helios-1/2); near 1 AU (Wind, ACE and STEREO-A/B); and from 1.35 to 5.4 AU (Ulysses). We also differentiate the IP shocks into two populations, those with a detected ICME and those without one. We find, as expected, that there are no significant differences in the results from spacecraft positioned at 1 AU. Moreover, the distributions of shock parameters, as well as the shock normal have no significant variations with the heliocentric distance. Additionally, we investigate how the number of shocks associated to stream-interaction regions (SIRs) increases with distance in proportion of ICME/shocks. From 1 to 5 AU, SIRs/ shock occurrence increases slightly from 21% to 34%, in contrast ICME/shocks occurrence decreases from 47% to 17%. We find also indication of an asymmetry induced by the Parker spiral for SIRs and none for ICMEs.

==> labels.tex <==

1 Section \ref{Sec:introduction}
2 Section \ref{Sec:selection}
   2.1 Section \ref{Sec:missions}
   2.2 Section \ref{Sec:databases}
   2.3 Section \ref {Sec:Ulysses}
3 Section \ref{Sec:1au}
   3.1 Section \ref{Sec:Comparing1au}
   3.2 Section \ref{Sec:WithWithoutICMEs}
   3.3 Section \ref{Sec:Angles}
         Equation \ref{EqLambda}
4 Section \ref{Sec:distances}
   4.1 Section \ref{Sec:Evolution_properties}
   4.2 Section \ref{Sec:Lambda}
   4.3 Section \ref{Sec:DistLambda}
5 Section \ref{Sec:Conclusion}

Appendix  \ref{Appendix:A}
Appendix  \ref{Appendix:B}
Appendix  \ref{Appendix:C}

 1 Figure \ref{UlyssesProfiles1}
 2 Figure \ref{Allshocks1AU_HistSW}
 3 Figure \ref{shocks1AU_HistSW}
 4 Figure \ref{1AU_HistSW_Corr}
 5 Figure \ref{fittPlot}
 6 Figure \ref{1AUToLamb}
 7 Figure \ref{lambdaDistributionsHelUly02}
 8 Figure \ref{MethComp}
 9 Figure \ref{LambdaComp}
10 Figure \ref{shocksHelUlyss_HistSW}

1 Table~\ref{table_1}
2 Table \ref{table_Ulysses}
3 Table \ref{table_icmes_1au}
4 Table \ref{table_ipshocks_icmes}


